TOI-908: a planet at the edge of the Neptune desert transiting a G-type star

We present the discovery of an exoplanet transiting TOI-908 (TIC-350153977) using data from TESS sectors 1, 12, 13, 27, 28 and 39. TOI-908 is a T = 10.7 mag G-dwarf ($T_{eff}$ = 5626 $\pm$ 61 K) solar-like star with a mass of 0.950 $\pm$ 0.010 $M_{\odot}$ and a radius of 1.028 $\pm$ 0.030 $R_{\odot}$. The planet, TOI-908 b, is a 3.18 $\pm$ 0.16 $R_{\oplus}$ planet in a 3.18 day orbit. Radial velocity measurements from HARPS reveal TOI-908 b has a mass of approximately 16.1 $\pm$ 4.1 $M_{\oplus}$ , resulting in a bulk planetary density of 2.7+0.2-0.4 g cm-3. TOI-908 b lies in a sparsely-populated region of parameter space known as the Neptune desert. The planet likely began its life as a sub-Saturn planet before it experienced significant photoevaporation due to X-rays and extreme ultraviolet radiation from its host star, and is likely to continue evaporating, losing a significant fraction of its residual envelope mass.

==> referee.tex <==
%% We would like to thank the referee for their careful reading of the manuscript and their suggested improvements.  We have implemented all the suggested corrections and changes. We have produced a new PDF manuscript with all amendments in yellow highlighted font.  We also list all the changes in detail below:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

GENERAL COMMENTS:
My main concern on the manuscript regards the determination of the stellar rotation period, which in turn drives the modeling of the planetary evolution. The first estimate of the rotation period of TOI-908 is presented in Sect. 3.2.2 as 20.53 days, coming from the measured projected rotational velocity vsini = 2.56+-0.64 km/s, and this is linked to the measured periodicity of 19.29 days in the RV periodogram. No, uncertainty is given on this first estimate of the rotation period, but in the following paragraph a Gaussian prior is adopted for the GP rotation-period hyper-parameter, as N(20.53,1.5). This standard deviation is not justified in the text, and appears very optimistic since the estimate of the rotation period comes from the rotational velocity which has a relative error of around 25\% (which should produce a comparable relative error on the rotation period, 20+-5 d). The result of the GP modeling appears to be the value Prot = 20.238+-1.312 days presented in Table 4 (although is not clearly stated), which troubles me, as the derived error appears very close to the standard deviation of the adopted (and not clearly motivated) prior, and thus does not look very reliable. Finally in Sect. 4.6, while discussing the evaporation history of the planet, the authors cite the rotation period as 20.27+-0.94 days, with a slightly different value and uncertainties which are not cited elsewhere in the manuscript. This is important, as the discussion of the evolution of the star is based on the measured rotation period. (see also comments on Fig. 14 below)
Moreover, the measurement of Prot appears to be only driven by the RV datasets, as the photometric modeling does not appear to include a rotational component (which is agreeable, since the photometric data shown in Fig. A2 do not show any rotational modulation). The authors mention in Sect. 2.3 several activity indicators they derived from the HARPS spectra of the target (some of which are also listed in Table 3), but in the analyses is never discussed whether the stellar rotation signal is present in these datasets. They analyses of the spectroscopic activity indexes might support a more precise and accurate measurement of Prot, which would in turn strengthen the evaporation modeling.

Another general comment I would like to make, is that I see the structure and evolution modeling as the main focus of the paper: the presence of a well-measured planet within the Neptunian-desert is very interesting due to its evolving nature, and thus this should be stressed out in the title and abstract (which mention only past evaporation, while the models suggest that the planet is still evolving), and discussed at length in the rest of the paper, as this planet present a very interesting candidate for transmission-spectroscopy observations, both from space and ground. Specific comments in this sense are provided below.

%% We have added the suggested phrasing to the abstract.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

SPECIFIC COMMENTS:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Abstract:

%% - The abstract should also mention on the potential internal structure of the planet, and highlight that the planet not only “experienced significant photoevaporation”, but most probably will continue evaporating losing a significant fraction of its residual envelope mass.

%% This statement has been amended to the abstract.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 1 Introduction:

%% - “the so-called ‘Neptune desert’ or ‘evaporation desert’ “ another common name is the ‘sub-Jovian desert’.

%% This change has been made.


%% - “The HARPS-NOMADS program (...) aims to significantly increase the number of planet confirmations in this parameter space...” please clarify exactly what do you mean by “this parameter space”, since it is unclear if it refers to the neptunian desert or more in general.

%% This has been updated to explicitly refer to the Neptune desert.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 2.3 HARPS radial velocity observations:

%% - please state the r.m.s. of the RV dataset, as well as the mean error.

%% This has been added.

%% - In Figure 4 and 5 can be seen at least 2 clear outliers in the RV time series. This could be taken out of the time series, after checking them with a 3-sigma cut, or with Chauvenet's criterion to confirm that they are in fact outliers. This could improve the RV fit of the data.

%% We have re-run our modelling, values and plotting with the two outlying points removed.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 3.1 Stellar analysis:

%% - Table 4: please list also the mean logR’hk among the stellar properties, in order to better frame its activity level.

%% The logR'hk values were not taken as measurements during the HARPS observations, the S-index values are either identical or derived from it. These values show a very marginal periodicity at 14.8 days and little else.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 3.2.1 Light curve detrending:

%%- please include explicitly the equation of the GP kernel adopted for the TESS photometry analysis.

%% We have added the corresponding equation for the GP kernel.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 3.2.2 Radial velocity (RV) detrending:

%% - “We first examine the HARPS radial velocity data using the DACE platform, in which we find two significant periodic signals above the level of the 1\% analytical FAP (False Alarm Probability) that are not aliases of each other.” please add here a reference to Figure 10, showing the RV data GLS periodogram.

%% This figure reference has been added.


%%- “We also calculate a rotational period of 20.53 days” please state the associated error to this period estimate.

%% We have added this error.


%% - “The prior for P rot is set up as a normal distribution around the predicted value of 20.53 days with a standard deviation of 1.5 days, based on the analysis from DACE.” discussed in GENERAL COMMENTS. Change the prior standard deviation to a physically motivated value, or adopt a uninformative constant prior. Since there is a 19d signal in the raw RVs, the GP regression should be able to recover the stellar rotation signal even without a informative prior.

%% We have updated our prior on the rotation period to be uniform, centered around 20.53 with a SD of 7 days, based on the calculated vsini errors. All resulting values from the new modelling run have been updated.


%% - As mentioned above, the addition  here of the analysis of the activity indicators derived from HARPS spectra (logR’hk, FWHM, etc) could provide additional evidence on the exact rotation period of the star, and could be used to train the GP and/or to derive a more physically motivated prior for the rotation period.

%% The logR'hk values were not taken as measurements during the HARPS observations, and the FWHM values are provided in Table 3 along with the value of the mean in Section 3.2.2.


%% - “We first find predicted values for the radial velocity of TOI-908 b at each data point in the HARPS data, and set a uniform prior between 0 and 10 m s −1 for the semi-amplitude K of the planet signal.” this sentence is not clear, please rephrase it.

%% This wording has been updated for clarity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 4 Results and discussion:

%% - please list in the beginning of this Section the derived radius and mass of the planet, to introduce the following discussion.

%% These values have been added to the section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 4.1 The Radius Valley:

%% - I think that this sub-section should be removed, as TOI-908b is not close to the valley, and thus this discussion is not really pertinent to the paper. Also can be confused to a reader not familiar with the radius valley, and neptunian desert, as they are similar but distinct feature of the parameter space.

%% The text and associated figure have been removed.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 4.4 Additional planets and TTVs:

%% - “We perform a BLS (Box Least Squares; Kovács et al. 2002) search on the TESS light curve data with the transit model for TOI-908 b subtracted, and find no evidence of additional significant signals above a False Alarm Probability (FAP) of 0.1 (Figure 10)” the referenced Figure shows the periodogram of the RV data, not the BLS of the TESS light-curve.

%% The reference to the figure has been removed.


%% - “We search the HARPS data using the DACE platform, which is capable of performing a periodogram search for additional periodic signals after the removal of the TOI-908 b radial velocity signal and the stellar rotation signal, and again we find no evidence for additional planets in the system.” It is not clear if the authors checked only the periodogram after removing the RV periodogram signal of TOI-908b (i.e. circular signal), or if they computed the residuals after removing the complete planetary signals as computed by the joint modeling. Please clarify (the latter is the most robust approach)

%% We removed the RV periodogram signal; this has been clarified in the text.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 4.5 Internal Structure modeling:

%% - “We thus solve a system of two equations: (1) the definition of envelope mass fraction shown in Equation 3, and (2) the envelope structure model by Chen & Rogers (2016), summarised in Equation 4:” this statement is a bit misleading, as Eq. 3 and 4 alone do not appear to form a solvable system of equation, since it would require at least the relation between Mcore and Rcore, since they both appear in the equations (although the previous sentence states that the only two unknown are fenv and Rcore. Please rephrase and clarify.

%% This has been rephrased and clarified.


%% - “We perform an additional study of the internal structure of the planet with a Bayesian analysis, using the derived stellar and planetary properties.” please provide a table listing the results of this model as Table 6 for the previous one, or add the results of the additional model to Table 6 for an easier comparison. The results of the two models should also be homogenized, as the first produces the Envelope mass fraction, while the second the fraction of the total radius represented by the atmosphere, and thus are not easily comparable.

%% We have added Table 7 to the manuscript for comparison between the two methods.


%% - Table 6: the uncertainty of the envelope mass fraction is listed as 0.022+-0.10, instead of +-0.010

%% This has been corrected.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 4.6 Evaporation history of the planet:

%% - “The underlying cause of evaporation is still under debate, though,” please provide some reference for alternative mechanisms. All the references provided in the previous sentence appear to assume photoevaporation as the cause of atmospheric evaporation.

%% References to this have been added.


%% - Figure 8: it would be interesting to highlight in the mass-radius diagram other planets that are inside the neptunian desert, to highlight eventual common properties.

%% We have added 4 additional planets to the diagram and labelled them accordingly, and altered the ranges of the axes for clarity.


%%- Figure 9: it could be interesting to show the age of the planets (whstellar rotation periods g starsen determined), e.g. as color-coding, to highlight whether the planets inside the desert are younger of the general population and if TOI-908b is older/younger than other nearby planets.

%% We assume that the referee is referring to Figure 8 here (Neptune desert), and we have elected not to include age estimates for similar planets as we have no evidence that these planets are young, and the individual age estimates are not well constrained. We hope that the additional planets on the graph provide some further context for the planet discovery and characterisation to the referee's satisfaction.


%% - “The rotation period of TOI-908 of 20.27 ± 0.94 days,” see general comments.

%% This has been corrected.


%% - It is unclear which age is used for the evolution study, as the age listed in Table 4 has large uncertainties, with a 1sigma interval going from 3 to 6 Gyr. This should be investigated further, as the issue of the discrepant rotation period with theoretical models could be explained taking into account the age uncertainty (maybe?). Moreover, in Figures 14 and 15, very small error bars are shown for the stellar age, in contrast with the value from Table 4. Where do these other uncertainties come from? From visual inspection of Figure 14, taking into account the 1.5Gyr uncertainty on the age could reconcile the apparent discrepancy between the rotation of TOI-908 and the theoretical prediction.

%% We have updated the plots with the correct age uncertainty.
%% We have pointed out that the lower error on the age is consistent with the model.


%% - From the main text and Figure 15, it appears that the simulations covered only the central value of envelope mass fraction listed in Table 6 (2.2\%), although its uncertainties are very large. It would be interesting to investigate other values within the uncertainties, to show how the evaporation history would change for lower/higher values of fenv that would still be compatible with the data.
%% Moreover, how would the results of the Bayesian structure model present in Section 4.5 change the evaporation history modeling? Would the conclusion on the initial radius and mass of the planet change? Would the future outcome of evaporation change?

%% We have re-run our simulations to model the evaporation history of both the gaseous planet as well as the water planet predicted by the Bayesian structure model. We have also modelled the spread in evaporation histories from the 1-sigma errors on the planet's mass, radius, and age.


%% - It could interesting to highlight in Figure 9 the evolution path of the planet according to the evaporation model, to show how evaporation “moves” the planet through the Neptunian desert.

%% Because Figure 8 is plotted in terms of period, which is an aspect that we do not model - therefore the evolutionary path is best presented in Figures 13 and 14. We hope that the additional planets on the graph provide some further context for the planet discovery and characterisation to the referee's satisfaction.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% 5 Conclusion:

%% - In addition to JWST follow-up, this target could also be interesting for spectroscopic evaporation measurement  via the metastable helium line with ground-based instruments such as CARMENES, NIRSPEC, GIANO, etc.

%% We have amended this statement to the conclusion. 

==> referee2.tex <==
%% We would like to thank the referee for their careful reading of the manuscript and their suggested improvements.  We have implemented all the suggested corrections and changes. We have produced a new PDF manuscript with all amendments in yellow highlighted font.  We also list all the changes in detail below:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Section 2.3:

%% - “...the standard activity indicators of S-index, Ha-index, Na-index, Ca-index and log(R’HK ).” This contradicts what said by the authors in two different replies to the previous comments, i.e. ‘The logR'hk values were not taken as measurements during the HARPS observations’. S-index and logR’hk can be derived from HARPS spectra, and in fact the latter is derived from the former correcting for photospheric and basal flux contributions, and is most commonly used as it allows comparison of activity levels across spectral types. This is why I previously suggested to add the median logR’hk value to the stellar parameters table, as it allows to evaluate the activity level of the star.

%% For this reason I wonder why  the Ha-index, Na-index, Ca-index and log(R’HK ) data are not listed in Table 3 along the other time series. Moreover, it is still not clear in the draft whether the activity data is used in the analyses or not. In the previous replies the authors stated generically that they find a marginal 14.8d periodicity in the S-index, This should be discussed in the text, together with the periodicities or lack of them found in the other indicators, as it is different from the measured rotation period of 20.53d, however the large error bars could make the two values compatible. Once again, since the stellar rotation drive the analysis of the evolution of the system, it should be studied as thoroughly as possible.

%% We have amended the text to reflect the measurements that were taken, added Figure 7 to represent the activity indicators shown in Table 3, and also added the periodograms for the remaining Ha, Na and Ca measurements in Appendix Figure A1, and their values in A5 - all new additions are referenced in-text and additional discussion has been added. After further examination we find the periodicities above the FAP lines are most likely to be related to the rotation period, which itself is relatively loosely constrained and degenerate with the inclination of the star.

%% Table 3: in addition to adding the other activity indicators discussed above, the table should also contain the uncertainties of all activity measurements.

%% We have added error columns to each of the columns in Table 3.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Section 3.2.1:

%% - Equation (1) is confusing, as presents a different notation than the just defined log(s2) , log(w0), and log(Sw4). Moreover S is written as a function of w, which is not present in the right-side of the equation where omega appears. Neither w nor omega are defined in the text.

%% We have updated the formatting of the equation and text to ensure consistency of notation.

%% Section 3.2.2:

%% - “RMS 0.0048, mean error 2.79 km s−1 )” it should be m/s, not km.

%% We have implemented this correction.

%% - “The prior for Prot is set up as a normal distribution around the predicted value of 20.53 days with a standard deviation of 1.5 days,” the SD should be 7 days, as listed in table A1. Also, please reference the prior Tables (A1-4) when discussing the corresponding analyses, or clarify in the text of Appendix A what is what, as it is not clear from the unreferenced tables.

%% We have corrected the values of the prior, and added a reference to the prior table.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Section 4.3:

%% - “besides the predicted rotation period of 19.29 days.” where does this prediction comes from? I understand that this value is inside the uncertainties of the Prot computed from the previous analysis, but this statement suggests that there is an indication of a rotation period of exactly 19.29 days, which is confusing.

%% We have updated the text here to reflect the true value, which should now be consistent throughout the text.

%%Section 4.4:

%%- “The case with water leads to an atmosphere representing 20\% of the total radius, whereas the case without water produces a thicker gaseous envelope of almost 35\% of the total radius.” this statement contradicts the values presented in Table 7, as for the water case 0.54 is not 20\% of 2.9+0.54, (16\%) nor for the dry case 1.02/(1.02+3.04) = 25\%. Moreover, the internal structure analysis presented in Table 7 appears in contradiction with the planetary radius derived from the transit analysis, as the total radius Rcore+Renv is different from the the Rp=3.186 value listed in Table 5 both in the water (3.44) and dry (4.06) cases. Although all these values have large uncertainties that make them almost compatible, it is still not clear why such different values are obtained. This problem does not appear to be present in the other structural analysis, as the Rcore and Renv values from Table 6 results in Rcore+Renv = 3.18, very close to Rp. Please correct and/or clarify this.

%% We have updated Table 7 and the text to reflect that the case with water actually leads to an atmosphere that is 18% of the total radius, not 20%. The modeled radii are 2.9 +- 0.47 and 3.04 +- 0.46, which no longer contradicts the radius derived from the transit analysis (3.186 Re).


==> referee3.tex <==
%% We would like to thank the referee for their careful reading of the manuscript and their suggested improvements.  We have implemented all the suggested corrections and changes. We have produced a new PDF manuscript with all amendments in yellow highlighted font.  We also list all the changes in detail below:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Section 2.3:
%% “We present the Lomb-Scargle periodograms of the parameters presented in Table 3” it should be data, or time series, instead of parameters.
%% “their values are presented in Appendix A1 and Appendix A5” please specify the reference to ‘Figure A1’ and ‘Table A5’

%% We have implemented these changes and updated the references accordingly.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Section 3.2.2:
%% “with a standard deviation of 7 days (Appendix A1)” again please specify ‘Table A1’

%% We have updated this reference.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Figure 7 (and other periodogram plots):
% “The False Alarm Probabilities (FAP) are marked as the horizontal grey lines at 0.1, 1 and 10\% from bottom to top.” it should be reversed, being 10\% the bottom FAP level and 0.1\% the top.

%% We have updated the figure caption to reflect this.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Table7:
%% The second column still list the incorrect variables “Rcore” and “Mcore”.

%% We have updated the variables to 'Rtot' and 'Mtot'.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Figure A1:
%% “Periodograms for the HARPS radial velocity data of the values presented in Appendix A1.” the periodograms shown are of the activity indices, not the radial velocities, and the reference to Appendix A1 is incorrect, should point to Table A5.

%% We have updated this reference and fixed the labeling of the FAP lines according to comments on Figure 7.
